NestedFormer: Nested Modality-Aware Transformer for Brain Tumor Segmentation

Multi-modal MR imaging is routinely used in clinical practice to diagnose and investigate brain tumors by providing rich complementary information. Previous multi-modal MRI segmentation methods usually perform modal fusion by concatenating multi-modal MRIs at an early/middle stage of the network, which hardly explores non-linear dependencies between modalities. In this work, we propose a novel Nested Modality-Aware Transformer (NestedFormer) to explicitly explore the intra-modality and inter-modality relationships of multi-modal MRIs for brain tumor segmentation. Built on the transformer-based multi-encoder and single-decoder structure, we perform nested multi-modal fusion for high-level representations of different modalities and apply modality-sensitive gating (MSG) at lower scales for more effective skip connections. Specifically, the multi-modal fusion is conducted in our proposed Nested Modality-aware Feature Aggregation (NMaFA) module, which enhances long-term dependencies within individual modalities via a tri-orientated spatial-attention transformer, and further complements key contextual information among modalities via a cross-modality attention transformer. Extensive experiments on BraTS2020 benchmark and a private meningiomas segmentation (MeniSeg) dataset show that the NestedFormer clearly outperforms the state-of-the-arts. The code is available at https://github.com/920232796/NestedFormer.

==> Tables/ablation_2.tex <==
\begin{table*}[t]
    \centering
    \caption{Ablation study for different modules on MeniSeg dataset.}
    \label{tab:ablation_result}
    \renewcommand\arraystretch{1.5}
    \setlength\tabcolsep{5pt}%调列距
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{c c c c c c c c c c c c c c}
    \hline
    Dataset & \multicolumn{11}{c}{MeniSeg}\\
    \hline
     & \multicolumn{3}{c}{Encoder} &  & \multicolumn{3}{c}{Fusion} &  & \multicolumn{3}{c}{Metric}\\
    \cline{2-4} \cline{6-8} \cline{10-12}
    Anatomy & CNN & PB & GPB &  &  TToA & TCA & Gate & & Tmuor & Edema & Avg\\
    % \cline{2-3} \cline{5-6} \cline{8-9} 
    % Metrics & Dice & HD95 &  & Dice & HD95 & & Dice & HD95 \\
    $baseline 1$ & \checkmark &  &  &  &  &  &  &  & 0.805 & 0.675 & 0.74 \\
    $baseline 2$ &  &  & \checkmark &  & \checkmark &  &  &  & 0.816 & 0.688 & 0.752 \\
    $baseline 3$  &  &  & \checkmark &  & \checkmark & \checkmark &  &  & 0.825 & \textbf{0.699} & 0.762 \\

    $baseline 4$ &  & \checkmark &  &  & \checkmark
    & \checkmark & \checkmark &  & 0.823 & 0.697 & 0.76 \\
    
    $baseline 5$ &  &  & \checkmark &  & \checkmark
    & \checkmark & \checkmark &  & \textbf{0.834} & 0.695 & \textbf{0.765}\\

    \hline
    
    \end{tabular} 
    }
\end{table*}



==> Tables/two_dataset_result.tex <==
\begin{table*}[t]
    \centering
    \caption{Comparison on BraTS 2020 and MeniSeg dataset.}
    \label{tab:two_dataset_result}
    \renewcommand\arraystretch{1.5}
    \setlength\tabcolsep{5pt}%调列距
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c c c c c c c c c  c c  c  c | c  c c c c c c c c}
    \hline
    Dataset & \multicolumn{11}{c}{BraTS2020} &  & \multicolumn{8}{c}{MeniSeg}\\
    \hline
    Anatomy & \multicolumn{2}{c}{WT} &  & \multicolumn{2}{c}{TC} & &  \multicolumn{2}{c}{ET} &  & \multicolumn{2}{c}{Avg} &  &  & \multicolumn{2}{c}{Tumor} &  & \multicolumn{2}{c}{edema} &  & \multicolumn{2}{c}{Avg}\\
    \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} \cline{15-16} \cline{18-19} \cline{21-22}
    Metrics & Dice & HD95 &  & Dice & HD95 & & Dice & HD95 & & Dice & HD95 & & & Dice & HD95 &  & Dice & HD95 & & Dice & HD95 \\
    \hline
    3D-UNet~\cite{cciccek20163d} & 0.902 & 2.929 &  & 0.762 & 5.100 &  & 0.658 & 7.780 &  & 0.774 & 5.269  & & & 0.799 & 5.099 &  & 0.676 & 9.655 &  & 0.737 & 7.377 \\
    SegResNet~\cite{myronenko20183d} & 0.910 & 1.419 &  & 0.774 & 3.569 &  & 0.663 & 6.324 &  & 0.782 & 3.770  & & & 0.813 & 2.970 &  & 0.665 & 10.438 &  & 0.739 & 6.704\\
    MAML~\cite{zhang2021modality} & 0.912 & 3.549 &  & 0.778 & 6.710 &  & 0.657 & 7.789 &  & 0.782 & 6.016  & & &  0.819 & 2.112 &  & 0.682 & 9.158 &  & 0.750 & 5.635\\
    \hline
    SwinUNet(2D)~\cite{cao2021swin} & 0.883 & 2.213 &  & 0.724 & 5.295 &  & 0.616 & 9.375 &  & 0.741 & 5.627  & & & 0.807 & 1.817 &  & 0.679 & 7.986 &  & 0.743 & 4.901\\
    TransBTS~\cite{wang2021transbts} & 0.889 & 2.181 &  & 0.763 & 3.847 &  & 0.679 & \textbf{5.113} &  & 0.777 & 3.713  & & & 0.809 & \textbf{1.742} &  & 0.679 & 6.388 &  & 0.744 & \textbf{4.065}\\
    UNETR~\cite{hatamizadeh2022unetr} & 0.908 & 2.768 &  & 0.772 & 4.477 &  & 0.677 & 6.845 &  & 0.785 & 4.696  & & & 0.818 & 3.279 &  & 0.693 & 7.837 &  & 0.755 & 5.813\\
    \hline
    Our method (LightMFT) & \textbf{0.914} & \textbf{1.113} &  & \textbf{0.786} & \textbf{3.446} &  & \textbf{0.704} & 5.480 &  & \textbf{0.801} & \textbf{3.346}  & & & \textbf{0.830} & 2.786 &  & \textbf{0.709} & \textbf{5.667} &  & \textbf{0.769} & 4.226\\
    \hline
    \end{tabular}
    }
\end{table*}


